A Multi-purpose Realistic Haze Benchmark with Quantifiable Haze Levels and Ground Truth

Imagery collected from outdoor visual environments is often degraded due to the presence of dense smoke or haze. A key challenge for research in scene understanding in these degraded visual environments (DVE) is the lack of representative benchmark datasets. These datasets are required to evaluate state-of-the-art vision algorithms (e.g., detection and tracking) in degraded settings. In this paper, we address some of these limitations by introducing the first realistic hazy image benchmark, from both aerial and ground view, with paired haze-free images, and in-situ haze density measurements. This dataset was produced in a controlled environment with professional smoke generating machines that covered the entire scene, and consists of images captured from the perspective of both an unmanned aerial vehicle (UAV) and an unmanned ground vehicle (UGV). We also evaluate a set of representative state-of-the-art dehazing approaches as well as object detectors on the dataset. The full dataset presented in this paper, including the ground truth object classification bounding boxes and haze density measurements, is provided for the community to evaluate their algorithms at: https://a2i2-archangel.vision. A subset of this dataset has been used for the ``Object Detection in Haze'' Track of CVPR UG2 2022 challenge at http://cvpr2022.ug2challenge.org/track1.html.

==> Response Letter/R1.tex <==
\section*{Reviewer 1:}

\subsection*{1. Approach}

\point{The proposed dataset seems more suited for benchmarking than for training. Because the corresponding hazy and haze-free images have differences in the underlying scene (as seen in Fig 1). For a dataset to be used in training, it should contain the image of a scene with and without the effect of haze. I could not understand how the haze-free images have been captured. I agree that capturing it is difficult, and the authors have used a method outlined in Sec III-C to find the best possible match.} \\
\re
Thanks for pointing this out. There are two concerns to be addressed here.
\begin{itemize}
    \item \textbf{A2I2-Haze more suitable for benchmarking than training?} We agree that A2I2-Haze is more suitable for benchmarking rather than for training, since the scene and object diversity is relatively limited. However, we also showed in the experiments by proper pretraining using existing UAV-based object detection datasets, our A2I2-Haze could still be used for training and achieve reasonable performance.
    \item \textbf{How to capture the (paired) haze-free images?} The haze-free and hazy images are paired at scene-level rather than pixel level. The pairing is achieved by well-designed data collection and offline matching. 
        \begin{itemize}
            \item Our UAV is flying in a lawn-mowing pattern based on pre-programmed gps coordinates (aka, waypoints). The flight plan for the collection was defined using a survey grid in Mission Planner to generate a cross-hatch pattern over a predefined area. The area was selected using an arbitrary rectangle within the Mission Planner, with the bounds of the rectangle selected to keep the area of interest within view of the cameras as much as possible over a range of altitudes. The survey grid was cross-hatched with a 10m lane spacing. In order to maintain consistency between altitudes, the survey grid was copied, and the altitude was increased in 5m increments from 15-50m. UAS was commanded to face toward the center of the grid at all points during its ﬂight. The GPS coordinate for the center of the grid was determined by the UAS by manually placing the UAS at the point of interest and using its GPS to determine the center of the grid. Please refer to Section III.A.1. for more details.
            \item We proposed a ``Coarse-to-Fine Matching'' strategy to achieve the scene-level pairing. Given two video sequences (hazy and haze free), we first cut each video into short clips of 2 seconds. We then manually selected hazy and haze-free clips that were similar at the scene level. Lastly, for each selected clip pair, we used ``Coarse-to-Fine Matching'' strategy to find the best pair-able frames with least amount of translation or rotation. Please refer to Algorithm 1 for more details.
        \end{itemize}
\end{itemize}
\hfill \break

\point{What is the idea behind finding the closest matching hazy and haze-free images, even though they can be different? The proposed approach can fail in the presence of dense haze.}   \\
\re
Thanks for pointing this out. There are two concerns to be addressed here.
\begin{itemize}
    \item \textbf{Goal of pairing hazy with the corresponding haze-free images.} The goal of pairing hazy with the corresponding haze-free images is to find the ground-truth haze-free image for the hazy image in training the dehazing model. Although our proposed Cycle-DehazeNet does not utilize the scene-level matched prior in the training, we release the dataset with paired hazy and haze-free images for future usage, e.g. progressively increase the dehazing difficulty by starting from paired samples.
    \item \textbf{Failure in dense haze for the proposed matching approach.} It is true that our proposed ``Coarse-to-Fine Matching'' would fail in the presence of dense haze. Due to UAV's high flying altitude and rapid movement speed, we sought scene-level matching rather than pixel-level matching. We manually check the returned paired hazy and haze-free images by the proposed ``Coarse-to-Fine Matching''. If it fails, we manually find best pairable images given the selected hazy and haze-free clips that were similar at the scene level. Such a final human intervention could guarantee the correctness even in the presence of dense haze.
\end{itemize}
\hfill \break

\point{The ``focusing'' part in the proposed cycle GAN based network is not clear.} \\
\re
Thank you for pointing this limitation out. We observe that the hazy areas in our dataset are mostly distributed around four corners instead of the central part. Based on that, we would like to force our proposed method to more focus on haze rather than clean parts. Thus the cropped four $512 \times 512$ patches from the corners of each image are used as ``focus'' (red bounding boxes in Fig. 9). We emphasize more on the hazy area than the whole image by assigning larger weights for the ``focus'' patch in the final loss. Please refer to Section IV.B.2. for more details.

\hfill \break

\point{Since the dataset is provided for the community, the expectation is the website will display some details of the dataset before requiring a login to get the data. But currently, the website requires a login before showing anything related to the dataset. (Priya et al.)} \\
\re
Thank for giving such a valuable suggestion. We will display some exemplar images of A2I2-Haze, with some brief explanation. Since the website is currently maintained by the IT department of DEVCOM U.S. Army Research Laboratory, the ETA of website update will be Feb 14th.

==> Response Letter/R2.tex <==
\section*{Reviewer 2:}

\point{The title might be confusing and needs to be corrected. Since the hazy scenes are generated using smoke generator this dataset is not a real one but a realistic dataset. Please update the title.} \\
\re 
Thanks for pointing this mistake out. We have updated the title by replacing ``real'' with ``realistic''. We have also done the replacement throughout the paper.
\hfill \break

\point{Also the abstract has to be updated: ``the first paired real image benchmark dataset with hazy and haze-free images'' is not completely true since NH-Haze and O-HAZE are datasets that use the same principles and have been introduced several years before.} \\
\re
Thank you for pointing this mistake out. We claim the proposed A2I2-Haze to the first realistic haze benchmark with the following two distinctions:
\begin{itemize}
    \item in-situ smoke measurement using ground sensors that are aligned to both aerial and ground imagery;
    \item paired hazy and haze-free imagery from both aerial and ground view.
\end{itemize}
We have updated the abstract to stress the distinctions.
\hfill \break

\point{It is not very clear how many different scenes have been recorded. It is only one scene recorded from different perspectives? How different are those 1033 pairs of images?} \\
\re
A2I2-Haze were captured in two separate settings – a) grass field as the background, and b) ground with concrete slabs as the background. For the aerial dataset, after each trial, target objects were re-positioned to generate different configuration of objects. The images with good pairing were then randomly isolated from the trials. However, the annotated ground dataset is only available from one configuration of target objects at this time.
\hfill \break

==> Response Letter/R3.tex <==
\section*{Reviewer 3:}

\point{Further elaboration is needed for the proposed Cycle-DehazeNet.} \\
\re 
Thanks for pointing this out. We have updated Section IV.B.2. to include more details. Cycle-DehazeNet has three major novelty points.
\begin{itemize}
    \item Cycle-DehazeNet introduces both cycle-consistency loss and perceptual loss.
    \item Cycle-DehazeNet could work on HR images by patch-level fusion. The reconstructed target pixel value using a weighted sum given by all the collided pixels from different patches.
    \item The cropped four $512 \times 512$ patches from the corners of each image is used as ``focus''. As the hazy area, the ``focus'' patches are assigned larger weights in the final loss.
\end{itemize}
\hfill \break

\point{How is the proposed Cycle-DehazeNet different from Cycle-Dehaze?} \\
\re
Both Cycle-DehazeNet and Cycle-Dehaze are inspired from Cycle-GAN. Our proposed Cycle-DehazeNet is different from Cycle-Dehaze in two aspects. 
\begin{itemize}
    \item Cycle-DehazeNet could work on HR images by patch-level fusion. Specifically, we first pad the input HR image from $1845 \times 1500$ to $2048 \times 1536$, so that the width and height are divisible by $512$. Then, we extract overlapping $512 \times 512$ patches at a stride of $256$. Last, the pixel value is computed as a weighted sum of all the collided pixels from different patches.
    \item Cycle-DehazeNet utilizes the prior of haze focus in A2I2-Haze's data collection. We observe that the hazy area is typically further away from the image center. The cropped four $512 \times 512$ patches from the corners of each image is used as ``focus''. As the hazy area, the ``focus'' patches are assigned larger weights in the final loss.
\end{itemize}

\hfill \break

\point{How to compute the final pixel value in the overlapped region from collided pixels?} \\
\re 
Thank for pointing the missed details out. We have updated the manuscript to include it. Since the overlapping $512 \times 512$ patches are extracted at a stride of $256$, a pixel in the high-resolution image may be covered by multiple patches, where the $i$-th patch produces a prediction $p_i$ of the target pixel. We hypothesize that the patches geometrically closer to the target pixel should carry more weights. Finally, we compute the reconstructed target pixel value $p_t$ using a weighted sum given by
\begin{equation}
    p_t = \frac{\sum_{i=1}^N w_i p_i}{\sum_{i=1}^N w_i},
\end{equation}
where $N$ is the number of patches that cover the subject pixel and $w$ follows a Gaussian distribution w.r.t. the geometric distance between the patch center and the target pixel.
\hfill \break

\point{Missed references for dehazing algorithms.} \\
\re
Thank you for providing the following missed references for dehazing algorithms. We have included them in Section II.A.
\begin{itemize}
    \item 4kDehazing~\cite{zheng2021ultra}: Ultra-High-Definition Image Dehazing via Multi-Guided Bilateral Learning, CVPR 2021.
    \item DW-GAN~\cite{fu2021dw}: A Discrete Wavelet Transform GAN for NonHomogeneous Dehazing, CVPR 2021 Workshop.
    \item \cite{shyam2021towards} Towards Domain Invariant Single Image Dehazing, AAAI 2021.
    \item MSRL-DehazeNet~\cite{yeh2019multi} Multi-Scale Deep Residual Learning-Based Single Image Haze Removal via Image Decomposition, TIP 2020.
    \item DM$^2$F-Net~\cite{deng2019deep} Deep Multi-Model Fusion for Single-Image Dehazing, ICCV 2019.
    \item LAP-Net~\cite{li2019lap}: Level-Aware Progressive Network for Image Dehazing, ICCV 2019.
\end{itemize}
\hfill \break

\point{Missed references for dehazing benchmarks.} \\
\re
Thank you for providing the following missed references for dehazing benchmarks. We have included them in Section II.B. Please also check Table 1 for detailed comparison.
\begin{itemize}
    \item MRFID~\cite{liu2020end}: End-to-End Single Image Fog Removal Using Enhanced Cycle Consistent Adversarial Networks, TIP 2020.
    \item BeDDE~\cite{zhao2020dehazing}: Dehazing Evaluation: Real-World Benchmark Datasets, Criteria, and Baselines, TIP 2020.
    \item Dense-Haze~\cite{ancuti2019dense}: A Benchmark for Image Dehazing with Dense-Haze and Haze-Free Images, ICIP 2019
\end{itemize}
\begin{table}[ht]
\caption{Properties of A2I2-Haze relative to other public dehazing benchmarks. Aer and Gr stands for aerial-view and ground-view, respectively. NH stands for non-homogeneous. HM stands for haze measurement. Details of A2I2-Haze is in the first paragraph of Section IV.}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Datasets}  &   \multicolumn{6}{c}{Attributes}  \\
\cline{2-7}
& Aer/Gr & In/Outdoor & NH & Syn/Real & \#Images & HM  \\
\hline
3R & G & O & & S & $2,750$ & \\
HazeRD & G & O & & S & $33$ & \\
O-Haze & G & O & & R & $45$ & \\
I-Haze & G & I & & R & $35$ & \\
4K & G & O & & S & $10,000$ & \\ 
REVIDE & G & I & & R & 1982 & \\
RESIDE & G & I+O & & S+R & $100,076$ & \\
BeDDE & G & O & & R & $208$ & \\
MRFID & G & O & & R & $800$ & \\
Dense-Haze & G & O & & R & $33$ & \\
NH-HAZE & G & O & \cmark & R & $55$ & \\
{\bf A2I2-Haze} & {\bf A+G} & {\bf O} & {\bf \cmark} & {\bf R} & {\bf 1,033} & {\bf \cmark} \\
\hline
\end{tabular}
}
\label{table:nonlin}
\end{table}
\hfill \break

\point{Writing and presentation} \\
\re
Thank you for pointing out the issues.
\begin{itemize}
    \item We have updated Fig.7 by increasing the text size for better readability.
    \item We have updated Fig.9 with the following modifications.
    \begin{itemize}
        \item We have merged the two VGGs into one, since the VGG is shared in Cycle-DehazeNet.
        \item We have updated all the subscripts. H2C means hazy to clean while C2H means clean to hazy. 
        \item We have updated the caption by replacing $G_A, G_B, D_A, D_B$ with $G_{H2C}, G_{C2H}, D_{clean}, D_{hazy}$.
        \item We have rewritten Section III.A, B, C and D to improve its readability.
    \end{itemize}
\end{itemize}

==> chapters/legacy.tex <==
\begin{table*}\normalsize
    \centering
    \caption{Vehicle Detection by UAV Using Off-the-shelf Detectors \zhenyu{Redraw with scatter point plots}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
         \multirow{2}*{Pretraining} & \multirow{2}*{Dehazing} & \multicolumn{3}{c|}{YOLOv5} & \multicolumn{3}{c|}{FasterRCNN} & \multicolumn{3}{c|}{CenterNet} & \multicolumn{3}{c}{YOLOX}\\
         \cline{3-14}
         ~ & ~ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR & $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ \\
         \hline
         \multirow{7}*{\textbf{VisDrone}} & hazy & 0.410 & 0.469 & 0.394 & 0.380 & 0.463 & 0.342 & 0.546 & 0.591 & 0.409 & 0.415 & 0.500 & 0.389\\
         \cline{2-14}
         ~ & GCANet      &    0.424    &  0.480   &   0.411 & 0.438 & 0.515 & 0.390 & 0.568 & 0.614 & 0.440 & 0.412 & 0.485 & 0.383 \\
        ~ & FFA-Net     &     0.402   &   0.455    &  0.383 & 0.395 & 0.461 & 0.346 & 0.557 & 0.560 & 0.397 & 0.416 & 0.497 & 0.387\\
        ~ & MSBDN    &    0.430  &    0.490   &   0.417 & 0.430 & 0.512 & 0.386 & 0.568 & 0.625 & 0.443 & 0.421 & 0.495 & 0.387 \\
        ~ & Trident      &    \textbf{0.503}  &    \textbf{0.574}   &   \textbf{0.482}   & \textbf{0.489} & 0.556 & \textbf{0.414}  & \textbf{0.596} & \textbf{0.678} & \textbf{0.486} & 0.383 & 0.432 & 0.333 \\
        ~ & SRKT     &    0.491  &    0.567   &   0.470  & 0.487 & 0.550 & 0.406 & 0.573 & 0.635 & 0.451 & 0.405 & 0.452 & 0.356 \\
        ~ & DWDehaze     &    0.487  &    0.547   &   0.466  & 0.445 & \textbf{0.568} & 0.395 &0.592 & 0.650 & 0.466 & \textbf{0.450} & \textbf{0.508} & \textbf{0.411}   \\
        \hline
        \multirow{7}*{\textbf{UAVDT}} & hazy & 0.099 & 0.117 & 0.096 & 0.216 & 0.264 & 0.196 & 0.493 & 0.457 & 0.323 & 0.296 & 0.325 & 0.256\\
        \cline{2-14}
        ~ & GCANet     &     0.142    &   0.176   &   0.139    & 0.245 & 0.310 & 0.222 & 0.520 & 0.503 & 0.361 & 0.279 & 0.295 & 0.224\\ 
        ~ & FFA-Net     &     0.115    &  0.138   &   0.113   & 0.218 & 0.149 & 0.181 & 0.506 & 0.457 & 0.326 & 0.299 & \textbf{0.328} & \textbf{0.256} \\ 
        ~ & MSBDN     &   0.145   &   0.176   &   0.145  & 0.240 & 0.301 & 0.219 & 0.520 & 0.510 & 0.363 & 0.288 & 0.307 & 0.240 \\  
        ~ & Trident     &     \textbf{0.198}   &   \textbf{0.242}    &   \textbf{0.188}    & \textbf{0.358} & \textbf{0.455} & \textbf{0.311} & \textbf{0.557} & 0.554 & 0.395 & 0.307 & 0.296 & 0.217 \\
        ~ & SRKT    &     0.166   &   0.207   &   0.163 & 0.299 & 0.384 & 0.268 & 0.541 & \textbf{0.570} & \textbf{0.402} & \textbf{0.309} & 0.280 & 0.214   \\
        ~ & DWDehaze     &    0.145  &    0.188   &   0.143   & 0.306 & 0.281 & 0.259 & 0.550 & 0.561 & 0.390 & 0.287 & 0.303 & 0.223  \\
        \hline
        \multirow{7}*{\textbf{UAVDT}+\textbf{VisDrone}} & hazy & 0.427 & 0.491 & 0.411 & 0.341 & 0.434 & 0.305 & 0.543 & 0.586 & 0.423 & 0.384 & 0.460 & 0.370\\
        \cline{2-14}
        ~ & GCANet     &     0.463    &   0.530   &   0.447  & 0.360 & 0.467 & 0.328 & 0.580 & 0.604 & 0.446 & 0.387 & 0.458 & 0.370  \\ 
        ~ & FFA-Net     &     0.439    &  0.498   &   0.418   & 0.359 & 0.424 & 0.302 & 0.551 & 0.579 & 0.418 & 0.382 & 0.456 & 0.366 \\ 
        ~ & MSBDN     &   0.466   &   0.541   &   0.452  & 0.392 & 0.504 & 0.354 & 0.571 & 0.627 & 0.456 & 0.379 & 0.450 & 0.364 \\  
        ~ & Trident     &     \textbf{0.533}   &   \textbf{0.626}    &   \textbf{0.510}    & 0.491 & 0.634 & 0.426 & 0.594 & \textbf{0.683} & \textbf{0.489} & 0.386 & 0.456 & 0.367\\
        ~ & SRKT    &     0.519   &   0.608   &   0.501 & \textbf{0.500} & \textbf{0.641} & \textbf{0.437} & 0.586 & 0.668 & 0.483 & 0.374 & 0.442 & 0.355 \\
        ~ & DWDehaze     &    0.504  & 0.580   &  0.487  & 0.489 & 0.621 & 0.420 & \textbf{0.596} & 0.671 & 0.484 & \textbf{0.431} & \textbf{0.506} & \textbf{0.410}   \\
        \hline
    \end{tabular}
    }
    \label{mAP comparison}
\end{table*}


\begin{table*}\normalsize
    \centering
    \caption{Vehicle Detection by UGV Using Off-the-shelf Detectors(Pretrained with CitySpace Dataset) \zhenyu{Redraw with scatter point plots}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
         \multirow{2}*{Dehazing} & \multicolumn{3}{c|}{YOLOv5} & \multicolumn{3}{c|}{FasterRCNN} & \multicolumn{3}{c|}{CenterNet} & \multicolumn{3}{c}{YOLOX}\\
         \cline{2-13}
         ~ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR & $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ \\
        \hline
        hazy & 0.233 & 0.286 & 0.220 & 0.449 & 0.544 & 0.392 & 0.573 & 0.651 & 0.460 & 0.205 & 0.266 & 0.191 \\
        \cline{1-13}
        GCANet     &  0.269  &  0.326    &    0.253   & \textbf{0.528} & \textbf{0.652} & \textbf{0.466} & 0.562 & 0.642 & 0.449 & 0.227 & 0.294 & 0.209\\ 
        FFA-Net     &   0.238      & 0.296     &    0.226  & 0.450 & 0.551 & 0.392 & 0.563 & 0.637 & 0.448 & 0.209 & 0.266 & 0.194 \\ 
        MSBDN     &   0.247   & 0.306     & 0.234    & 0.474 & 0.580 & 0.413 & 0.571 & 0.629 & 0.447 & 0.217 & 0.275 & 0.202 \\  
        Trident     &   \textbf{0.338}    &  \textbf{0.416}     &     \textbf{0.320}  & 0.524 & 0.644 & 0.461 & \textbf{0.576} & \textbf{0.682} & \textbf{0.472} & \textbf{0.309} & \textbf{0.393} & \textbf{0.283} \\
        SRKT    &    0.261    & 0.325     & 0.247   & 0.519 & 0.643 & 0.457 & 0.558 & 0.656 & 0.456 & 0.299 & 0.384 & 0.275   \\
        DWDehaze     & 0.240  & 0.306   &   0.227   & 0.481 & 0.599 & 0.425 & 0.575 & 0.678 & 0.465 & 0.273 & 0.364 & 0.250  \\
        \hline
    \end{tabular}
    }
    \label{ugv_detection }
\end{table*}


\begin{table*}\normalsize
    \centering
    \caption{Vehicle Detection by UAV After Dehazing}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
         \multirow{2}*{Dehazing} & \multicolumn{3}{c|}{YOLOv5} & \multicolumn{3}{c|}{FasterRCNN} & \multicolumn{3}{c|}{CenterNet} & \multicolumn{3}{c}{YOLOX}\\
         \cline{2-13}
         ~ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR & $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ \\
        \hline
        hazy & .427+\blue{.022} & .491+\blue{.047} & .411+\blue{.017} & .341+\blue{.07} & .434+\blue{.119} & .305+\blue{.076} & .543+\blue{.066} & .586+\blue{.107} & .423+\blue{.091} & .384+\blue{.028} & .460+\blue{.039} & .370+\blue{.025}\\
        \cline{1-13}
        GCANet     &     .463+\blue{.046}    &   .530+\blue{.067}   &   .447+\blue{.043}    & .360+\blue{.113} & .467+\blue{.144} & .328+\blue{.107} & .580+\blue{.073} & .604+\blue{.148} & .446+\blue{.111} & .387+\blue{.018} & .458+\blue{.021} & .370+\blue{.015}\\ 
        FFA-Net     &     .439+\blue{.014}    &  .498+.\blue{.035}   &   .418+\blue{.011}   & .359+\blue{.065} & .424+\blue{.120} & .302+\blue{.072} & .551+\blue{.067} & .579+\blue{.117} & .418+\blue{.097} & .382+\blue{.024} & .456+\blue{.029} & .366+\blue{.020} \\ 
        MSBDN     &   .466+\blue{.029}   &   .541+\blue{.047}   &   .452+\blue{.023}  & .392+\blue{.081} & .504+\blue{.124} & .354+\blue{.082} & .571+\blue{.071} & .627+\blue{.098} & .456+\blue{119} & .379+\blue{.048} & .450+\blue{.038} & .364+\blue{.026} \\  
        Trident     &     .533+\blue{.029}   &   .626+\blue{.047}    &   .510+\blue{.024}    & .491+\blue{.060} & .634+\blue{.082} & .426+\blue{.071} & .594+\blue{.061} & .683+\blue{.090} & .489+\blue{.081} & .386+\blue{.015} & .456+\blue{.027} & .367+\blue{.017} \\
        SRKT    &     .519+\blue{.005}   &   .608+\blue{.027}   &   .501-\blue{ .002} & .500+\blue{.007} & .641+\blue{.016} & .437+\blue{.021} & .586+\blue{.043} & .668+\blue{.073} & .483+\blue{.059} & .374+\blue{.020} & .442+\blue{.017} & .355+\blue{.015}   \\
        DWDehaze     &    .504+\blue{.042}  &    .580+\blue{.075}   &   .487+\blue{.033}   & .489+\blue{.042} & .621+\blue{.056} & .420+\blue{.064} & .596+\blue{.059} & .671+\blue{.092} & .484+\blue{.081} & .431+\blue{.010} & .506+\blue{.010} & .410+\blue{.008}  \\
        \hline
    \end{tabular}
    }
    \label{tab:detection_dehaze}
\end{table*}


\begin{table*}\normalsize
    \centering
    \caption{Vehicle Detection by UGV After Dehazing}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
         \multirow{2}*{Dehazing} & \multicolumn{3}{c|}{YOLOv5} & \multicolumn{3}{c|}{FasterRCNN} & \multicolumn{3}{c|}{CenterNet} & \multicolumn{3}{c}{YOLOX}\\
         \cline{2-13}
         ~ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR &  $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ & AR & $\text{AP}_{0.5}$ & $\text{AP}_{0.5:0.95}$ \\
        \hline
        hazy & .233+\blue{.132} & .286+\blue{.169} & .220+\blue{.122} & .449+\blue{.029} & .544+\blue{.036} & .392+\blue{.051} & .573-\blue{.044} & .651+\blue{.042} & .460+\blue{.019} & 0.205+\blue{.035} & 0.266+\blue{.021} & 0.191+\blue{.018} \\
        \cline{1-13}
        GCANet     &  .269+\blue{.113}  &  .326+\blue{.149}    &    .253+\blue{.107}   & .528+\blue{.017} & .652+\blue{.024} & .466+\blue{.034} & .562-\blue{.021} & .642+\blue{.088} & .449+\blue{.044} & 0.227+\blue{.075} & 0.294+\blue{.043} & 0.209+\blue{.038}\\
        FFA-Net     &   .238+\blue{.135}      & .296+\blue{.169}     &    .226+\blue{.124}  & .450+\blue{.031} & .551+\blue{.029} & .392+\blue{.051} & .563-\blue{.042} & .637+\blue{.048} & .448+\blue{.023} & 0.209+\blue{.032} & 0.266+\blue{.020} & 0.194+\blue{.014} \\ 
        MSBDN     &   .247+\blue{.124}   & .306+\blue{.149}     & .234+\blue{.113}    & .474+\blue{.027} & .580+\blue{.029} & .413+\blue{.051} & .571-\blue{.038} & .629+\blue{.068} & .447+\blue{.037} & 0.217+\blue{.103} & 0.275+\blue{.087} & 0.202+\blue{.076} \\  
        Trident     &   .338+\blue{.086}    &  .416+\blue{.118}     &     .320+\blue{.082}  & .524+\blue{.014} & .644+\blue{.021} & .461+\blue{.034} & .576-\blue{.034} & .682+\blue{.045} & .472+\blue{.016} & 0.309+\blue{.041} & 0.393+\blue{.034} & 0.283+\blue{.028} \\
        SRKT    &    .261+\blue{.138}    & .325+\blue{.170}     & .247+\blue{.122}   & .519+\blue{.017} & .643+\blue{.015} & .457+\blue{.033} & .558-\blue{.024} & .656+\blue{.060} & .456+\blue{.031} & 0.299+\blue{.058} & 0.384+\blue{.046} & 0.275+\blue{.039}   \\
        DWDehaze     & .240+\blue{.124}  & .306+\blue{.149}   &   .227+\blue{.115}   & .481+\blue{.025} & .599+\blue{.021} & .425+\blue{.041} & .575-\blue{.057} & .678+\blue{.001}& .465-\blue{.006} & 0.273+\blue{.027} & 0.364+\blue{.019} & 0.250+\blue{.014}  \\
        \hline
    \end{tabular}
    }
    \label{finetune comparison}
\end{table*}
